The Effect of Spatial Coupling on Compressive Sensing

Recently, it was observed that spatially-coupled LDPC code ensembles approach the Shannon capacity for a class of binary-input memoryless symmetric (BMS) channels. The fundamental reason for this was attributed to a "threshold saturation" phenomena derived by Kudekar, Richardson and Urbanke. In particular, it was shown that the belief propagation (BP) threshold of the spatially coupled codes is equal to the maximum a posteriori (MAP) decoding threshold of the underlying constituent codes. In this sense, the BP threshold is saturated to its maximum value. Moreover, it has been empirically observed that the same phenomena also occurs when transmitting over more general classes of BMS channels. In this paper, we show that the effect of spatial coupling is not restricted to the realm of channel coding. The effect of coupling also manifests itself in compressed sensing. Specifically, we show that spatially-coupled measurement matrices have an improved sparsity to sampling threshold for reconstruction algorithms based on verification decoding. For BP-based reconstruction algorithms, this phenomenon is also tested empirically via simulation. At the block lengths accessible via simulation, the effect is quite small and it seems that spatial coupling is not providing the gains one might expect. Based on the threshold analysis, however, we believe this warrants further study.

==> definition.tex <==
%---------------------------------------------------------------------------------
% temporary options:
% comments and corrections when writing
%---------------------------------------------------------------------------------
\definecolor{TODO}{rgb}{0.6,0.6,0.6} % TO DO!!!!
\newcommand{\todo}[1]{{\color{TODO}TO DO: {#1}}\marginpar{\color{TODO}$\leftarrow$ TO DO!}}
\definecolor{TOCHECK}{rgb}{0.8,0.8,0.8} % TO CKECK!!!!
\newcommand{\tocheck}[1]{\marginpar{\color{TOCHECK}$\leftarrow$ TO CHECK: {#1}}}
%---------------------------------------------------------------------------------


%---------------------------------------------------------------------------------
% LaTex environment
%---------------------------------------------------------------------------------
\newtheorem{theorem}{Theorem}
\newcommand{\btheo}{\begin{theorem}}
\newcommand{\etheo}{\end{theorem}}
\newcommand{\bproof}{\begin{proof}}
\newcommand{\eproof}{\end{proof}}
\newtheorem{definition}[theorem]{Definition}
\newcommand{\bdefi}{\begin{definition}}
\newcommand{\edefi}{\end{definition}}
\newtheorem{fact}[theorem]{Fact}
\newcommand{\bprop}{\begin{fact}}
\newcommand{\eprop}{\end{fact}}
\newtheorem{corollary}[theorem]{Corollary}
\newcommand{\bcor}{\begin{corollary}}
\newcommand{\ecor}{\end{corollary}}
\newtheorem{example}[theorem]{Example}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}
\newtheorem{lemma}[theorem]{Lemma}
\newcommand{\blemma}{\begin{lemma}}
\newcommand{\elemma}{\end{lemma}}
\newtheorem{remark}[theorem]{Remark}
\newcommand{\bremark}{\begin{remark}}
\newcommand{\eremark}{\end{remark}}
\newtheorem{conj}[theorem]{Conjecture}
\newcommand{\bconj}{\begin{conj}}
\newcommand{\econj}{\end{conj}}
\newtheorem{observation}{Observation}
%---------------------------------------------------------------------------------


%---------------------------------------------------------------------------------
% Mathematics:
%---------------------------------------------------------------------------------
%---------> international notations
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\naturals}{\ensuremath{\mathbb{N}}}
\newcommand{\integers}{\ensuremath{\mathbb{Z}}}
%---------> mynotations
\newcommand{\expectation}{\ensuremath{\mathbb{E}}}
\newcommand{\argmin}{\ensuremath{\text{argmin}}}
\newcommand{\defas}{\ensuremath{\stackrel{{\vartriangle}}{=}}} 
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
%{\ensuremath{\stackrel{\triangle}{=}}}%{\ensuremath{:=}}%{\colon=}}  %\stackrel{\vartriangle}{=}
%---------------------------------------------------------------------------------


%---------------------------------------------------------------------------------
% Coding and Information Theory:
%---------------------------------------------------------------------------------
%---------> Modulation (transmitted bit)
\def\0{{\tt 0}} % Ex.: BPSK modulation => 0 is encoded into +1
\def\1{{\tt 1}} % Ex.: BPSK modulation => 1 is encoded into -1
\def\?{{\tt *}} % erasure symbol
\def\g{{\tt g}} % guess symbol
\newcommand{\gp}{\ensuremath{\gamma}} % proba for guessing a bit
\newcommand{\chm}[1]{\ensuremath{{{\mu^{{\tt{\epsilon}}}_{#1}}}}} % 
%\def\chm{{\tt {z} }} % channel message
\newcommand{\lrm}[1]{\ensuremath{{{\mu^{{\tt{x}}}_{#1}}}}} % left-to-right message
\newcommand{\rlm}[1]{\ensuremath{{{\mu^{{\tt{y}}}_{#1}}}}} % right-to-left message
\newcommand{\m}{\ensuremath{{{\mu}}}} % message
\def\lra{{\tt {x}}} % left-to-right density
\def\rla{{\tt {y}}} % right-to-left density
%---------> LDPC and Turbo notations
\newcommand{\graph}{{\ensuremath{\tt G}}}
%\newcommand{\code}{{\ensuremath{\tt C}}}
\newcommand{\ldpc}{{{\ensuremath{\text{LDPC}}}}}
\newcommand{\ddp}{dd~pair~} %degree distribution pair %d.d.
\newcommand{\maxwell}{M~} %Maxwell
%\DeclareMathOnperator{\ldpc}{LDPC}
\DeclareMathOperator{\w}{w}    % weight
%\DeclareMathOperator{\graph}{G}
\newcommand{\n}{\ensuremath{n}} % code length
\newcommand{\drate}{r} % design rate
\newcommand{\rate}{\ensuremath{R}} % design rate
\newcommand{\ledge}{\ensuremath{\lambda}} % ledge (edge perspective) 
\newcommand{\redge}{\ensuremath{\rho}} % redge (edge perspective
\newcommand{\lnode}{\ensuremath{\Lambda}} % lnode (node perspective) 
\newcommand{\rnode}{\ensuremath{\Gamma}} % rnode (node perspective) 
\newcommand{\ldegree}{{\ensuremath{\ensuremath{\tt l}}}} % left degree (regular codes) 
\newcommand{\rdegree}{{\ensuremath{\ensuremath{\tt r}}}} % right degree (regular codes) 
%---------> EXIT quantities, thresholds and channel
\newcommand{\ih}{\ensuremath{{\tt{h}}}} % intrinsic (or input or channel) entropy
\newcommand{\cp}{\epsilon} % channel parameter 
\newcommand{\xh}{\ensuremath{h}} % extrinsic (or EXIT) entropy
\newcommand{\ML}{\ensuremath{\text{ML}}} % Maximum Likelihood
\newcommand{\MAP}{\ensuremath{\text{MAP}}} % Maximum A Posteriori
\newcommand{\LMAP}{\ensuremath{\text{LMAP}}} % Maximum A Posteriori
\newcommand{\BP}{\ensuremath{\text{BP}}} % Belief Propagation 
\newcommand{\Galsmall}{\ensuremath{\text{\tiny Gal}}} % Belief Propagation 
\newcommand{\EBP}{\ensuremath{\text{EBP}}} % Extended Belief Propagation
\newcommand{\Sh}{\ensuremath{\text{Sh}}} % Shannon
\newcommand{\SC}{\ensuremath{\text{SC}}} % Stability Condition
\newcommand{\MLsmall}{\ensuremath{\text{\tiny ML}}} % Maximum Likelihood
\newcommand{\MAPsmall}{\ensuremath{\text{\tiny MAP}}} % Maximum A Posteriori
\newcommand{\LMAPsmall}{\ensuremath{\text{\tiny LMAP}}} % Maximum A Posteriori
\newcommand{\BPsmall}{\ensuremath{\text{\tiny BP}}} % Belief Propagation
\newcommand{\Shasmall}{\ensuremath{\text{\tiny Sha}}} % Belief Propagation
\newcommand{\GalBsmall}{\ensuremath{\text{\tiny GalB}}} % Belief Propagation
\newcommand{\MPsmall}{\ensuremath{\text{\tiny MP}}} % Belief Propagation
\newcommand{\LMPsmall}{\ensuremath{\text{\tiny LMP}}} % Belief Propagation
\newcommand{\EBPsmall}{\ensuremath{\text{\tiny EBP}}} % Extended Belief Propagation
\newcommand{\Shsmall}{\ensuremath{\text{\tiny Sh}}} % Shannon
\newcommand{\SCsmall}{\ensuremath{\text{\tiny SC}}} % Stability Condition
\newcommand{\itersmall}{{\tiny \text{$\ell$}}} % 
\newcommand{\iter}{\ell} % 

%\newcommand{\iteration}{\ensuremath{\ell}} % iteration index during BP iterative decoding

\newcommand{\xl}{\ensuremath{{\tt{x}}}}%\xi}} %decoding parameter, FIND A LETTER FOR IT!!!
                                              % = left EXIT entropy
\newcommand{\xr}{\ensuremath{{\tt{y}}}}%\xi}} % rexit or right EXIT entropy
\newcommand{\lxl}{\ensuremath{\underline{\xl}}} %lower parameter
\newcommand{\uxl}{\ensuremath{\overline{\xl}}} %upper parameter
%--- non-math-mode macros
\newcommand{\exitentropy}{EXIT~} %EXIT entropy 

\newcommand{\qed}{{\hfill \footnotesize $\blacksquare$}}
\renewcommand{\mid}{\,|\,}
\newcommand{\tablespace}{\vspace{10pt}}
\newcommand{\dens}[1]{\mathsf{#1}}
\newcommand{\Ldens}[1]{\dens{#1}}
\newcommand{\absdens}[1]{\absd{\dens{#1}}}
\newcommand{\absLdens}[1]{\absdens{#1}}
\newcommand{\Ddens}[1]{\mathfrak{{#1}}}
\newcommand{\BEC}{\ensuremath{\text{BEC}}}
\newcommand{\EC}{\ensuremath{\text{EC}}}
\newcommand{\BSC}{\ensuremath{\text{BSC}}}
\newcommand{\BAWGNC}{\ensuremath{\text{BAWGNC}}}
\newcommand{\BMS}{\ensuremath{\text{BMS}}}
\newcommand{\BM}{\ensuremath{\text{BM}}}
\newcommand{\BSCsmall}{\ensuremath{\text{\tiny BSC}}}
\newcommand{\BMSsmall}{\ensuremath{\text{\tiny BMS}}}
\newcommand{\BECsmall}{\ensuremath{\text{\tiny BEC}}}
\newcommand{\BAWGNCsmall}{\ensuremath{\text{\tiny BAWGNC}}}

\newcommand{\absd}[1]{|#1|}
\newcommand{\absDdens}[1]{\absd{\Ddens{#1}}}
\newcommand{\absDdist}[1]{\absd{\mathfrak{#1}}}
\newcommand{\Ldensities}{$L$-densities}
\newcommand{\Ddensities}{$D$-densities}
\newcommand{\Gdensities}{$G$-densities}


\newcommand {\bE} {\mathbb{E}}
\newcommand {\gn} {\Omega}
\newcommand {\bt} {\tilde{\beta}}
\newcommand {\bad} {\mathcal{B}}
\newcommand {\newbad} {\Delta\mathcal{B}}
\newcommand {\marked} {\mathcal{M}}
\newcommand {\bound} {\mathcal{B}}
\newcommand {\leaves} {\mathcal{L}}
\newcommand {\newleaves} {\Delta \mathcal{L}}
\newcommand {\good} {\mathcal{G}}
\newcommand {\nb} {\mathcal{N}}
\newcommand {\expn} {\mathcal{X}}
\newcommand{\errors}{{\ensuremath{\tt E}}}
\newcommand {\itn} {i}
\newcommand {\I} {\mathbb{I}}
\newcommand {\mcE} {\mathcal{E}}
\newcommand {\mts} {\textbf{s}}
\newcommand {\mtS} {\textbf{S}}
\newcommand {\mtT} {\textbf{T}}
\newcommand {\mtt} {\textbf{t}}
\newcommand {\var} {\mathcal{V}}
\newcommand {\chset} {\mathcal{C}}
\newcommand {\pml} {p_{-1}^{(\ell)}}
\newcommand {\ppl} {p_{+1}^{(\ell)}}
\newcommand {\ppi} {p_{+1}^{(0)}}
\newcommand {\pmi} {p_{-1}^{(0)}}
\newcommand {\mbN} {\underline{N}}
\newcommand {\msgspace} {\mathcal{M}}
\newcommand {\msg} {\mu}

\newcommand{\cset}[1]{{\mathcal C}^{({#1})}}
\newcommand{\cs}{{\mathcal C}^{(0)}}
\newcommand{\vs}[1]{{\mathcal V}^{(0)}_{#1}}
\newcommand{\csn}{{\mathcal C}^{(1)}}
\newcommand{\vsn}[1]{{\mathcal V}^{(1)}_{#1}}

%\newcommand{\csnum}{|{\mathcal C}^{(0)}|}
%\newcommand{\vsnum}[1]{|{\mathcal V}_{#1}^{(0)}|}
%\newcommand{\csnnum}[1]{|{\mathcal C}_{#1}^{(1)}|}
%\newcommand{\vsnnum}[1]{|{\mathcal V}_{#1}^{(1)}|}
\newcommand{\csnum}{c^{(0)}}
\newcommand{\vsnum}[1]{v_{#1}^{(0)}}
\newcommand{\csnnum}[1]{c_{#1}^{(1)}}
\newcommand{\vsnnum}[1]{v_{#1}^{(1)}}
\newcommand{\dr}{d_r}
\newcommand{\dl}{d_l}
\newcommand{\dlh}{\hat{d}_l}
\newcommand {\badold} {\mathcal{B}_{\iter}}
\newcommand {\badnew} {\mathcal{B}_{\iter+1}}
\newcommand {\badoldonly} {\mathcal{B}_{\iter} \setminus \mathcal{B}_{\iter+1}}
\newcommand {\badnewonly} {\mathcal{B}_{\iter+1} \setminus \mathcal{B}_{\iter}}
\newcommand {\nofbadoldonly} {\mathcal{C}}
\newcommand {\nofbadnewonly} {\mathcal{D}}
\newcommand {\nofbadoldandnew} {\mathcal{T}}
\newcommand {\badcup} {\mathcal{U}}
\newcommand {\badcap} {\mathcal{I}}
\newcommand {\badcupnum} {u}
\newcommand {\badcapnum} {i}
\newcommand {\badoldnum} {b}
\newcommand {\badnewnum} {b'}
\newcommand {\edge} {{\mathtt e}}
\newcommand {\vnode} {{\mathtt v}}
\newcommand {\cnode} {{\mathtt c}}
\newcommand {\rootnode} {r}
\newcommand {\T} {\mathcal{T}}
\newcommand {\M} {\mathcal{M}}
\newcommand {\Mt} {{\mathcal{M}}}
\newcommand{\E}{{\ensuremath{\tt E}}}
\newcommand {\erasureset} {U}
\newcommand {\ev}[1]{\mathcal{{#1}}}
\newcommand {\init} {\mathcal{I}}
\newcommand{\treeensemble}{{\mathcal T}} 
\newcommand{\eldpc}[3]{\text{LDPC}\left(#1, #2, #3 \right)}
\newcommand{\LGalBsmall}{\ensuremath{\text{\tiny LGalB}}}
\newcommand{\GBsmall}{\ensuremath{\text{\tiny GB}}}
\newcommand{\LMSsmall}{\ensuremath{\text{\tiny LMS}}}
\newcommand{\MSsmall}{\ensuremath{\text{\tiny MS}}}
\newcommand{\LQMSsmall}{\ensuremath{\text{\tiny LQMS}}}
\newcommand{\QMSsmall}{\ensuremath{\text{\tiny QMS}}}
\newcommand{\EEx}{\hfill $\Diamond$}
\newcommand{\EDe}{\hfill $\Diamond$}
\DeclareMathOperator{\perr}{\mathfrak{E}}
\newcommand {\badedgeset} {\mathcal{B}}
\newcommand {\touched} {\mathcal{M}}
\newcommand {\ntouched} {{M}}
\newcommand {\witness} {\mathcal{W}}
\newcommand {\errorset} {\mathcal{E}}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indicator}[1]{\ind_{\{ #1 \}}}
\newcommand{\gensemble}[1]{\mathcal{G}(#1)}
\newcommand{\expander}{\mathcal{X}}
\newcommand{\iiter}{\ell_0} % 
\newcommand{\de}[1] {x_{#1}}
\newcommand{\vb}{{\mathtt v}}
\newcommand{\ck}{{\mathtt c}}
\newcommand{\bY}{\bar{Y}}
\newcommand{\bX}{\bar{X}}
\newcommand{\by}{\bar{y}}
\newcommand{\bx}{\bar{x}}
\newcommand{\gibbs}{\mu}
\newcommand{\nbd}{{\mathcal N}}
\newcommand {\varset} {\mathcal{V}}
\newcommand {\edgeset} {\mathcal{E}}
\newcommand {\negx} {\tilde{x}}
\DeclareMathOperator{\batta}{\mathfrak{B}}      % Bhattacharya operator
\newcommand{\code}[1]{\mathtt{C}^{#1}}
\newcommand{\exponent}{\mathtt{E}}
\newcommand{\dmin}{\mathtt{dmin}}
\newcommand{\GF}{\text{GF}}
\renewcommand{\dh}{{{d_{H}}}}
%\newcommand{\xstab}{x_{\text{s}}}
%\newcommand{\ystab}{y_{\text{s}}}
%\newcommand{\xustab}{x_{\text{u}}}
%\newcommand{\yustab}{y_{\text{u}}}
\newcommand{\xBP}{x_{\text{BP}}}


% EXIT Charts
% -----------
\newcommand{\exitf}{h}
\newcommand{\exitF}{H}


==> definitions.tex <==
% The following commands allow CVS to insert the
% current information regarding this file:
% ----------------------------------------------
% $RCSfile$
% $Date: 2008-12-10 08:02:24 -0700 (Wed, 10 Dec 2008) $
% $Author: ruediger $
% $Revision: 200 $
% $Source$
% $State$
% -----------------------------------------------
% Commands for theorems and such
% ------------------------------
%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{corollary}{Corollary}[chapter]
%\newtheorem{lemma}{Lemma}[chapter]
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{example}{Example}[chapter]
%\newtheorem{proposition}{Proposition}[chapter]
%\newtheorem{conjecture}{Conjecture}[chapter]
%\newtheorem{fact}{Fact}[chapter]
%\theoremstyle{definition}
%\newtheorem{exercise}{}[chapter]
\newcommand{\Exercises}{\section*{\centering Exercises}\addcontentsline{toc}{section}{\numberline{}Exercises}\markright{\footnotesize EXERCISES}}
\newcommand{\History}{\section*{\centering Notes}\addcontentsline{toc}{section}{\numberline{}Notes}\markright{\footnotesize NOTES}}
\newcommand{\btheorem}{\begin{theorem}\rm}
\newcommand{\etheorem}{\end{theorem}}
\newcommand{\bcorollary}{\begin{corollary}\rm}
\newcommand{\ecorollary}{\end{corollary}}
\newcommand{\bconjecture}{\begin{conjecture}\rm}
\newcommand{\econjecture}{\end{conjecture}}
\newcommand{\blemma}{\begin{lemma}\rm}
\newcommand{\elemma}{\end{lemma}}
\newcommand{\bdefinition}{\begin{definition}\rm}
\newcommand{\edefinition}{\end{definition}}
\newcommand{\bexample}{\begin{example}\rm}
\newcommand{\eexample}{\end{example}}
\newcommand{\bproposition}{\begin{proposition}\rm}
\newcommand{\eproposition}{\end{proposition}}
\newcommand{\bfact}{\begin{fact}\rm}
\newcommand{\efact}{\end{fact}}
\newcommand{\bexercise}{\begin{exercise}\rm}
\newcommand{\eexercise}{\end{exercise}}
\newcommand{\EEx}{\hfill $\Box$}
\newcommand{\EDe}{\hfill $\clubsuit$}

% algebraic objects
%------------------
\DeclareMathOperator{\reals}{\ensuremath{\mathbb{R}}}
\DeclareMathOperator{\realsplus}{\ensuremath{\mathbb{R}^+}}
\DeclareMathOperator{\creals}{\ensuremath{\bar{\mathbb{R}}}}
\DeclareMathOperator{\cR}{\creals}
\DeclareMathOperator{\crealsplus}{\ensuremath{\bar{\mathbb{R}}^+}}
\DeclareMathOperator{\cRp}{\crealsplus}
\DeclareMathOperator{\GF}{GF}
\DeclareMathOperator{\field}{\ensuremath{\mathbb{F}}}
\DeclareMathOperator{\F}{\field}
\DeclareMathOperator{\extensionfield}{\ensuremath{\mathbb{E}}}
\DeclareMathOperator{\semiring}{\ensuremath{\mathbb{K}}}
\DeclareMathOperator{\complex}{\ensuremath{\mathbb{C}}}
\DeclareMathOperator{\integers}{\ensuremath{\mathbb{Z}}}
\DeclareMathOperator{\naturals}{\ensuremath{\mathbb{N}}}
\DeclareMathOperator{\rationals}{\ensuremath{\mathbb{Q}}}

% operators 
% ---------
\DeclareMathOperator{\expectation}{\ensuremath{\mathbb{E}}} % expectation operator
%\DeclareMathOperator{\probability}{{\text{\rm P}}}    % alias
\DeclareMathOperator{\prob}{{\text{\rm P}}}    % generic probability
\DeclareMathOperator{\perr}{\mathfrak{E}}       % probability of error operator
\DeclareMathOperator{\batta}{\mathfrak{B}}      % Battacharya operator
\DeclareMathOperator{\fourier}{\mathfrak{F}}    % Fourier transform operator
\DeclareMathOperator{\harddec}{\mathfrak{H}}    % hard decision operation
\DeclareMathOperator{\w}{w}    % weight 


% generic code 
% ------------
\newcommand{\codeword}{{codeword}}
\newcommand{\dd}{dd} % degree distribution
\newcommand{\code}{C}
\newcommand{\dualcode}{C^{\perp}}
\newcommand{\generator}{G}
\newcommand{\parity}{H}
\newcommand{\gshannon}{{\cal G}}
\newcommand{\hshannon}{{\cal H}}
\newcommand{\capacity}{\text{C}}
\newcommand{\entropy}{\text{H}}

% Tanner graph 
% ------------
\newcommand{\graph}{{{\tt G}}}
\newcommand{\standardgraph}{\Gamma}
\newcommand{\standardgraphensemble}{{G}}
\newcommand{\complexgraph}[3]{{\cal G}_{#1}(#2, #3)}
\newcommand{\cnode}{{\tt c}}
\newcommand{\vnode}{{\tt v}}
\newcommand{\dr}{{\tt r}}
\newcommand{\dravg}{{\tt r}_{\text{avg}}}
\newcommand{\drmin}{{\tt r}_{\text{min}}}
\newcommand{\drmax}{{\tt r}_{\text{max}}}
\newcommand{\dl}{{\tt l}}
\newcommand{\dlavg}{{\tt l}_{\text{avg}}}
\newcommand{\dlmin}{{\tt l}_{\text{min}}}
\newcommand{\dlmax}{{\tt l}_{\text{max}}}
\newcommand{\Edges}{E}
\newcommand{\edge}{{{\tt e}}}
\newcommand{\codetensor}{f}
\newcommand{\hamiltonian}{E}

% algebraic notions
% -----------------
\newcommand{\group}{G}
\newcommand{\groupelement}{g}
\newcommand{\dualgroup}{\Gamma}
\newcommand{\character}{\gamma}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indicator}[1]{\ind_{\{ #1 \}}}
%\newcommand{\defeq}{\stackrel{\vartriangle}{=}}
\newcommand{\defeq}{\triangleq}
\newcommand{\myscriptsize}{\tiny}

% Tree codes 
% ----------
\newcommand{\treeensemble}{{\cal T}}
\newcommand{\ctreeensemble}{{\cal C}}
\newcommand{\nodetreeensemble}{\dot{\cal T}}
\newcommand{\edgetreeensemble}{\vec{\cal T}}
\newcommand{\nodectreeensemble}{\dot{\cal C}}
\newcommand{\edgectreeensemble}{\vec{\cal C}}
\newcommand{\tree}{{{\tt T}}}
\newcommand{\ltree}{{{\tt L}}}
\newcommand{\rtree}{{{\tt R}}}
\newcommand{\minimal}{{{\cal P}}}

% LDPC ensembles 
% --------------
\newcommand{\ensemble}[3]{{\cal C}\left(#1, #2, #3 \right)}
\newcommand{\nldpc}[2]{\text{LDPC}\left(#1, #2 \right)}
\newcommand{\eldpc}[3]{\text{LDPC}\left(#1, #2, #3 \right)}
\newcommand{\peldpc}[4]{\text{LDPC}\left(#1, #2, #3, #4 \right)}
\newcommand{\nsldpc}[2]{\text{LDPC}_{<}\left(#1, #2 \right)}
\newcommand{\esldpc}[3]{\text{LDPC}_{<}\left(#1, #2, #3 \right)}
\newcommand{\nrldpc}[2]{\text{LDPC}_{\circ}\left(#1, #2 \right)}
\newcommand{\erldpc}[3]{\text{LDPC}_{\circ}\left(#1, #2, #3 \right)}
\newcommand{\ldpcp}[2]{\text{LDPC}_{P}\left(#1, #2 \right)}
\newcommand{\ldpc}[3]{\text{LDPC}\left(#1, #2, #3 \right)}
\newcommand{\epldpc}[3]{\text{LDPC}_{P}\left(#1, #2, #3\right)}
\newcommand{\npldpc}[2]{\text{LDPC}\left(#1, #2 \right)}
\newcommand{\ledge}{\lambda}           % left degree distribution-edge perspective
\newcommand{\redge}{\rho}              % right degree distribution-edge perspective
%\newcommand{\densredge}[1]{\Gamma^{-1}(\redge(\Gamma(#1)))}
\newcommand{\densredge}[1]{\redge(#1)} % density form with Gamma dropped
\newcommand{\lnode}{\Lambda}           % left degree distribution-node perspective
\newcommand{\lnodenormalized}{L}           % left degree distribution-node perspective and normalized
\newcommand{\lnoden}{\lnodenormalized}     % left degree distribution-node perspective and normalized
\newcommand{\rnode}{P}                 % right degree distribution-node perspective
\newcommand{\rnodenormalized}{R}                 % right degree distribution-node perspective normalized
\newcommand{\rnoden}{\rnodenormalized}                 % right degree distribution-node perspective normalized
%\newcommand{\ledger}{\underline{\lambda}}           % left degree distribution-edge perspective
%\newcommand{\redger}{\underline{\rho}}              % right degree distribution-edge perspective
%\newcommand{\lnoder}{\underline{\Lambda}}           % left degree distribution-node perspective
%\newcommand{\rnoder}{\underline{P}}                 % right degree distribution-node perspective
\newcommand{\ddeq}{\circeq}                % equalilty of degree distributions in different representations

\newcommand{\ledger}{\lambda}           % left degree distribution-edge perspective
\newcommand{\redger}{\rho}              % right degree distribution-edge perspective
\newcommand{\lnoder}{\Lambda}           % left degree distribution-node perspective
\newcommand{\rnoder}{P}                 % right degree distribution-node perspective
\newcommand{\redgedev}{\delta}              % right degree distribution-edge perspective
\newcommand{\rnodedev}{\Delta}                 % right degree distribution-node perspective
\newcommand{\redgedom}{\gamma}              % right degree distribution-edge perspective
\newcommand{\rnodedom}{\Gamma}                 % right degree distribution-node perspective

\newcommand{\CtoV}{{\tt left-to-right }}
\newcommand{\VtoC}{{\tt right-to-left }}

% iterative decoder 
% -----------------
\newcommand{\iterations}{\ell}
\newcommand{\iteration}{\ell}
\newcommand{\erasureset}{{\cal E}}
\newcommand{\eset}{{\cal E}}
\newcommand{\kset}{{\cal K}}

% EXIT Charts
% -----------
\newcommand{\exitf}{h}
\newcommand{\exitF}{H}

% stopping sets etc. 
% ------------------
\newcommand{\total}{T}
\newcommand{\Total}{{\cal T}}
\newcommand{\stopping}{S}
\newcommand{\none}{N}
\newcommand{\None}{{\cal N}}
\newcommand{\bad}{B}
\newcommand{\Bad}{{\cal B}}
\newcommand{\ssmin}{s_{\text{min}}}
\newcommand{\ssmax}{s_{\text{max}}}
\newcommand{\ssmaximal}{s}

% mbs channels 
% ------------
\newcommand{\channelto}[1]{\xrightarrow{\quad #1 \quad}}
\newcommand{\smallchannelto}[1]{\xrightarrow{\; #1 \;}}
\newcommand{\channelfrom}[1]{\xleftarrow{\quad #1 \quad}}
\newcommand{\inalphabet}{{\cal X}} % channel input alphabet 
\newcommand{\out}{{\cal Y}}        % chanel output alphabet
\newcommand{\llr}{l}   % log-likelihood ratio
\newcommand{\Llr}{L}   % log-likelihood ratios as a rv
\newcommand{\diffp}{D}   % log-likelihood ratios as a rv
\newcommand{\delinf}{\Delta_{\infty}}  % delta function at infinity
\newcommand{\delzero}{\Delta_{0}}      % delta function at zero
%\newcommand{\conv}{\otimes}
\newcommand{\conv}{\star}
\newcommand{\physicallypreceeds}{\prec}
\newcommand{\physicallysucceeds}{\succ}

% density and distribution macros
%------------------
%\newcommand{\channel}[1]{\mathit{\MakeLowercase{#1}}}
\newcommand{\channel}[1]{\MakeLowercase{#1}}
\newcommand{\abs}[1]{{\lvert #1 \rvert}}
\newcommand{\absd}[1]{|#1|}
\newcommand{\spaceofLdistributions}{{\cal A}_{L}}
\newcommand{\spaceofabsLdistributions}{{\cal A}_{\absd{L}}}
\newcommand{\spaceofDdistributions}{{\cal A}_{D}}
\newcommand{\spaceofabsDdistributions}{{\cal A}_{\absd{D}}}
\newcommand{\spaceofGdistributions}{{\cal A}_{G}}
\newcommand{\Ddistribution}{$D$-distribution}
\newcommand{\absDdistribution}{$\absd{D}$-distribution}
\newcommand{\Ldistribution}{$L$-distribution}
\newcommand{\absLdistribution}{$\absd{L}$-distribution}
\newcommand{\Gdistribution}{$G$-distribution}
\newcommand{\Ddistributions}{$D$-distributions}
\newcommand{\absDdistributions}{$\absd{D}$-distributions}
\newcommand{\Ldistributions}{$L$-distributions}
\newcommand{\Gdistributions}{$G$-distributions}
\newcommand{\absGdistribution}{$\absd{G}$-distribution}
\newcommand{\absLdistributions}{$\absd{L}$-distributions}
\newcommand{\Ldensity}{$L$-density}
\newcommand{\absLdensity}{$\absd{L}$-density}
\newcommand{\Ddensity}{$D$-density}
\newcommand{\Gdensity}{$G$-density}
\newcommand{\absDdensity}{$\absd{D}$-density}
\newcommand{\absDdensities}{$\absd{D}$-densities}
\newcommand{\Ldensities}{$L$-densities}
\newcommand{\Ddensities}{$D$-densities}
\newcommand{\Gdensities}{$G$-densities}
\newcommand{\absLdensities}{$\absd{L}$-densities}
\newcommand{\vect}[1]{{\underline{#1}}}
\newcommand{\vectbs}[1]{{\underline{#1}}}

% generic distributions and densities
\newcommand{\dist}[1]{\mathsf{\MakeUppercase{#1}}}
\newcommand{\absdist}[1]{\absd{\dist{#1}}}
\newcommand{\dens}[1]{\mathsf{\MakeLowercase{#1}}}
\newcommand{\absdens}[1]{\absd{\dens{#1}}}
\newcommand{\heaviside}{\dist{H}}             % heaviside function
\newcommand{\ddist}[1]{\,d \dist{#1}}  % distribution
\newcommand{\vLdens}[1]{\underline{\dens{#1}}} % vector of densities
% L distributions and densities
\newcommand{\Ldist}[1]{\dist{#1}}
\newcommand{\absLdist}[1]{\absdist{#1}}
\newcommand{\Ldens}[1]{\dens{#1}}
\newcommand{\absLdens}[1]{\absdens{#1}}
% D distributions and densities
\newcommand{\Ddist}[1]{\mathfrak{\MakeUppercase{#1}}}
\newcommand{\absDdist}[1]{\absd{\mathfrak{\MakeUppercase{#1}}}}
\newcommand{\Ddens}[1]{\mathfrak{\MakeLowercase{#1}}}
\newcommand{\absDdens}[1]{\absd{\Ddens{#1}}}
% G distributions and densities
\newcommand{\Gdist}[1]{\mathit{\MakeUppercase{#1}}}
\newcommand{\absGdist}[1]{\absd{\mathit{\MakeUppercase{#1}}}}
\newcommand{\Gdens}[1]{\mathit{\MakeLowercase{#1}}}
\newcommand{\absGdens}[1]{\absd{\Ddens{#1}}}

% other stuff
\newcommand{\pdiff}{d}
\newcommand{\lgpdiff}{g}
\newcommand{\gmap}{\Gamma}
\newcommand{\Pdiff}{D}

% for proof of physical degradation theorem
\newcommand{\ugf}{u_{\text{\myscriptsize GF}}}
\newcommand{\ufg}{u_{\text{\myscriptsize FG}}}
\newcommand{\Afg}{A_{\text{\myscriptsize FG}}}
\newcommand{\Agf}{A_{\text{\myscriptsize GF}}}
\newcommand{\zAgf}{\hat{A}_{\text{\myscriptsize GF}}}
\newcommand{\zpm}{z_{\uparrow}}
\newcommand{\invzpm}{z^{-1}_{\uparrow}}
\newcommand{\invF}{{\absDdist{F}}^{-1}}
\newcommand{\invG}{{\absDdist{G}}^{-1}}

% picture macros
%
\newcommand{\nudge}[3]{\hspace{#1 pt}\raisebox{#2 pt}{#3}}
% junk macros 
% -----------
\newcommand{\sfield}{{\cal F}}
\newcommand{\dneigh}[2]{{\cal N}_{#1}^{#2}}
\newcommand{\rec}{{\tt r}}
\newcommand{\neigh}[2]{{\cal N}_{#1}^{#2}}
\newcommand{\gf}{\hat{\gamma}}
\newcommand{\sset}{{\cal S}}
\newcommand{\lset}{{\cal V}}
\newcommand{\rset}{{\cal C}}
\newcommand{\vset}{{\cal V}}
\newcommand{\e}{e}
\newcommand{\mue}{\mu}
\newcommand{\nue}{\nu}
\DeclareMathOperator{\degreefunction}{{\cal D}}
\DeclareMathOperator{\normalizeddegreefunction}{{\cal N}}
\newcommand{\tindex}{t}
\newcommand{\outp}{y}
\newcommand{\inp}{{\tt x}}
\newcommand{\cnd}{{\tt c}}
\newcommand{\mesg}{\mu}
\newcommand{\vnd}{{\tt v}}
%\newcommand{\vnd}[1]{\vnode_{#1}}
\def\Plo{\vnd_{\ell-1}}
\def\Rlo{\cnd_{\ell-1}}
\newcommand{\vnodes}{{{\cal V}}}
\newcommand{\cnodes}{{{\cal C}}}
\newcommand{\allone}{\vect{1}}
\newcommand{\oa}{{\cal O}}
\newcommand{\ma}{{\cal M}}
\newcommand{\node}{{\tt u}}
%\newcommand{\vmessagemap}[1]{\Psi_{\tt v}^{(#1)}}
%\newcommand{\cmessagemap}[1]{\Psi_{\tt c}^{(#1)}}
\newcommand{\vmessagemap}[1]{\Psi^{(#1)}}
\newcommand{\cmessagemap}[1]{\Phi^{(#1)}}
\newcommand{\prvmessagemap}[1]{{{}^\star\Psi}_{\tt v}^{(#1)}}
\newcommand{\prcmessagemap}[1]{{{}^\star\Psi}_{\tt c}^{(#1)}}
\newcommand{\oquan}{{q_o}}
\newcommand{\quan}{q}
\newcommand{\x}{{\tt x}}
\newcommand{\p}[2]{p_{#1}^{(#2)}}
\newcommand{\dedge}{\vec{\tt e}}
\newcommand{\q}[2]{q_{#1}^{(#2)}}
\newcommand{\vmsgmap}{\Psi_{\tt v}}
\newcommand{\cmsgmap}{\Psi_{\tt c}}
\newcommand{\mesn}[1]{\vnode_{#1}}
\newcommand{\chen}[1]{\cnode_{#1}}
\newcommand{\sign}{\ensuremath{\mathsf{sgn}\,}}
\newcommand{\simplegraph}{{\cal G}}
\newcommand{\prcmsgmap}{{{}^\star\Psi}_{\tt c} }
\newcommand{\prvmsgmap}{{{}^\star\Psi}_{\tt v} }
\DeclareMathOperator{\fnode}{{\tt f}}
\DeclareMathOperator{\unode}{{\tt u}}
\DeclareMathOperator{\gnode}{{\tt g}}
\DeclareMathOperator{\edges}{E}
\DeclareMathOperator{\neighbors}{N}
\newcommand{\correct}{{\cal G}}
\newcommand{\erroneous}{{\cal B}}
\newcommand{\pth}[1]{\left( #1 \right)}
\newcommand{\iterlim}{{\stackrel{\iteration \rightarrow \infty}{\longrightarrow}}}

% reed solomon codes
\newcommand{\spa}{A}
\newcommand{\spb}{B}
\newcommand{\spc}{C}
\newcommand{\chord}{S}

% stability paper
\newcommand{\ptree}{t}
\newcommand{\primsubtrees}{\Psi (T)}
\newcommand{\vnoderoot}{{\tt v}_{\text{\small root}}}
\newcommand{\droot}{d_{\text{\small root}}}
\newcommand{\smvnoderoot}{{\tt v}_{\text{\tiny root}}}
%\newcommand{\smprec}{P_{\text{\small rec}}}
%\newcommand{\perr}{\prob_{\text{\small err}}}
\newcommand{\tg}{\tilde{g}}
\renewcommand{\th}{\beta}
%\newcommand{\qleaf}{q_{\cal Q}}

\newcommand{\alphabet}{{\cal A}}
\newcommand{\alphabetsize}{A}
\def\llim{\lim_{x \rightarrow -\infty}}
\def\rlim{\lim_{x \rightarrow +\infty}}
\def\infpm{(-\infty,+\infty]}
\newcommand{\dominant}{{\cal D}}
\newcommand{\intlambda}{\text{$\int \!\! \lambda$}\;}
\newcommand{\intrho}{\text{$\int \!\! \rho$}\;}
\newcommand{\xzs}{\underline{x_0^{*}}}
\newcommand{\intrhomin}{\underline{\text{$\int \!\! \rho$}}\;}
\newcommand{\lambdatwomax}{\overline{\lambda_2}}
\newcommand{\intrhomax}{\overline{\text{$\int \!\! \rho$}}\;}
\newcommand{\ovi}{{\textstyle \frac{1}{i}}}
\newcommand{\ovip}{{\textstyle \frac{1}{i+1}}}
\newcommand{\ccns}{\text{$\int \!\! \lambda$}\;}
\newcommand{\ovj}{{\textstyle \frac{1}{j}}}
\newcommand{\ic}{\left(\ovi-\ccns\right)}
\newcommand{\omrji}{(1-r)^{j-i}}
\newcommand{\omr}{(1-r)}
\newcommand{\rji}{r^{j-i}}
\newcommand{\cip}{\left(\ccns-\ovip\right)}
\newcommand{\cj}{\left(\ccns-\ovj\right)}
\newcommand{\omrjip}{(1-r)^{j-i+1}}
\newcommand{\rjip}{r^{j-i+1}}
\def\Q{\text{$\cal Q$}}
\newcommand{\intrhomint}{\underline{\text{$\int \!\! \tilde{\rho}$}}\;}
\newcommand{\wst}{{\tt t}}
\newcommand{\wsv}{{\tt v}}
\newcommand{\centert}{{\tt T}}
\newcommand{\centerv}{{\tt V}}

\def\pl{x_\ell} % erasure probability at l-th round of BP on Erasure
                % Channel
\def\plo{x_{\ell-1}}
\def\Pl{\vnd_\ell} % Density of the messages sent from variable nodes to
                % check nodes at l-th round of the BP
\newcommand{\Rl}{a} % Density of messages sent from check nodes to
\newcommand{\distPl}{\int\!\vnd_{\ell}} % Density of the messages sent from variable nodes to
\newcommand{\distRl}{\int\! \cnd_{\ell}} % Density of messages sent from check nodes to
\newcommand{\distRlo}{\int\! \cnd_{\ell-1}}
\def\atanh{\mathrm{atanh}}
\def\vn{variable node}
\def\cn{check node}
\def\sgn{\mathrm{sgn}}

\def\L{\mathrm{L}} % \L(y) is the likelihood ratio of y

\def\indass{{\em independence assumption}}
%\def\BP{{\em belief-propagation}}

\newcommand{\mydeltat}{e}
\newcommand{\mydeltas}{c}
\newcommand{\mysigma}{d}
\newcommand{\mytau}{f}
\newcommand{\deltat}{\Delta t}
\newcommand{\deltas}{\Delta s}
\newcommand{\tdrift}{\text{f}_{t}}
\newcommand{\sdrift}{\text{f}_{s}}
\newcommand{\tvariance}{\text{f}_{t,t}}
\newcommand{\svariance}{\text{f}_{s,s}}
\newcommand{\tsvariance}{\text{f}_{t,s}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\infpm{(-\infty,+\infty]}
\def\llim{\lim_{x \rightarrow -\infty}}
\def\rlim{\lim_{x \rightarrow +\infty}}
\def\lgsgn{\sgn}
\def\mvc{{\tt m}_{\tt vc}} % Message sent from variable node v to check node c
\def\mvcl{\mvc^{(\ell)}}
\def\mvcl{\mvc^{(\ell)}}
\def\mcv{{\tt m}_{\tt cv}} % Message sent from check node c to variable node v
\def\mcvl{\mcv^{(\ell)}}
\def\scv{s_{cv}} % Sign
%\def\dx{\,\d x}
%\def\dy{\,\d y}
%\def\dz{\,\d z}
\def\dx{{\, d \! x}}
\def\dy{{\, d \! y}}
\def\dz{{\, d \! z}}
\def\dpp{{\, d \! p}}
\def\deps{{\, d \! \epsilon}}
\def\tensor{\star}
%\newcommand{\delinf}{\Delta_{\infty}}
\def\distRl{\int\! \cnd_{\ell}} % Density of messages sent from check nodes to
\def\distRlo{\int\! \cnd_{\ell-1}}
\def\distPl{\int\!\vnd _\ell} % Density of the messages sent from variable nodes to
                % check nodes at l-th round of the BP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% turbo code section
\newcommand{\demaps}[3]{\Gamma_{#3}^s(#1, #2)}  % map between densities for trellis: sytematic bits
\newcommand{\demapp}[3]{\Gamma_{#3}^p(#1, #2)}  % map between densities for trellis: parity bits
\newcommand{\demap}[3]{\Gamma_{#3}(#1, #2)}  % map between densities for trellis: either
\newcommand{\demapsshort}[2]{\Gamma^s(#1, #2)}  % map between densities for trellis: sytematic bits
\newcommand{\demappshort}[2]{\Gamma^p(#1, #2)}  % map between densities for trellis: parity bits
\newcommand{\demapshort}[2]{\Gamma(#1, #2)}  % map between densities for trellis: either
\newcommand{\iw}{i}   % input weight; weight of systematic bits
\newcommand{\ow}{o}   % output weight; weight of parity bits
\newcommand{\tw}{w}   % weight of all bits; total weight
\newcommand{\state}{\sigma}   % state of a trellis, i.e., content of shift register 
\newcommand{\State}{\Sigma}   % same as state but if considered as random variable 
\newcommand{\gfc}{C}   % generating function for weight distribution: convolutional code 
\newcommand{\gfp}{P}   % generating function for weight distribution: parallel concatenated code 
\newcommand{\gfs}{S}   % generating function for weight distribution: serially concatenated code
\newcommand{\gfpasym}{\bar{P}}   % generating function for weight distribution: parallel concatenated code
\newcommand{\gfsasym}{\bar{S}}   % generating function for weight distribution: serially concatenated code
\newcommand{\gfpasymp}{\tilde{P}}   % generating function for weight distribution: parallel concatenated code
\newcommand{\gfsasymp}{\tilde{S}}   % generating function for weight distribution: serially concatenated code
\newcommand{\cgfc}{c}   % coefficient of generating function for weight distribution: convolutional code
\newcommand{\cgfp}{p}   % coefficient of generating function for weight distribution: parallel concatenated code
\newcommand{\cgfs}{s}   % coefficient of generating function for weight distribution: serially concatenated code
\newcommand{\gfdet}{D}   % generating function of detours
\newcommand{\cgfpasym}{\bar{p}}   % coefficient of generating function for weight distribution: parallel concatenated code
\newcommand{\cgfsasym}{\bar{s}}   % coefficient of generating function for weight distribution: serially concatenated code
\newcommand{\cgfpasymp}{\tilde{p}}   % coefficient of generating function for weight distribution: parallel concatenated code
\newcommand{\cgfsasymp}{\tilde{s}}   % coefficient of generating function for weight distribution: serially concatenated cod
\newcommand{\mat}{M}   % matrix for transfer matrix method 
\newcommand{\matfinal}{\bar{M}}   % matrix for transfer matrix method for the last m steps
\newcommand{\matdet}{M^{\bullet}}   % matrix for transfer matrix method to compute detours 


\newcommand {\barr}{\begin{array}}
\newcommand {\earr}{\end{array}}

% covariance evolution
\newcommand{\ebar}{\overline{\epsilon}}
\newcommand{\Sur}{P_{\rm S}}
\newcommand{\Wh}{\widehat{W}}
\newcommand{\Xh}{\widehat{X}}
\newcommand{\Ph}{\widehat{P}}
\newcommand{\oX}{\overline{X}}
\newcommand{\oz}{\overline{z}}
\newcommand{\oth}{\overline{\theta}}
\newcommand{\fh}{\hat{f}}
\newcommand{\Dh}{\widehat{D}}
\newcommand{\Wt}{\widetilde{W}}
\newcommand{\Hp}{{\mathbb H}_+}
\newcommand{\R}{{\mathbb R}}
\newcommand{\vD}{\vec{\Delta}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vX}{\vec{X}}
\newcommand{\vz}{\vec{z}}
\newcommand{\Ai}{{\rm Ai}}
\newcommand{\Bi}{{\rm Bi}}
\newcommand{\ve}{\varepsilon}
%\newcommand{\ledger}{\lambda}           % left degree distribution-edge perspective
%\newcommand{\redger}{\rho}              % right degree distribution-edge perspective
%\newcommand{\lnoder}{\Lambda}           % left degree distribution-node perspective
%\newcommand{\rnoder}{P}                 % right degree distribution-node perspective
%\newcommand{\redgedev}{\delta}              % right degree distribution-edge perspective
%\newcommand{\rnodedev}{\Delta}                 % right degree distribution-node perspective
%\newcommand{\redgedom}{\gamma}              % right degree distribution-edge perspective
%\newcommand{\rnodedom}{\Gamma}                 % right degree distribution-node perspective
\newcommand{\xl}{x_{l}}
\newcommand{\xr}{x_{r}}
\newcommand{\xleft}{x_{l}}
\newcommand{\xright}{x_{r}}

% Macros from Changyan
\newcommand{\ensembleldpc}[3]{{\cal C}_{\text{LDPC}}(#1,#2, #3)}
\newcommand{\expurgatedensembleldpc}[4]{{\cal C}^{ex}_{\text{LDPC}}(#1,#2, #3,#4)}
\newcommand{\separateensembleldpc}[4]{{\cal C}^{#4<}_{\text{LDPC}}(#1,#2, #3)}
\newcommand{\ensembleldpcstatphys}[3]{{\cal C}^{\text{sp}}_{\text{LDPC}}(#1,#2, #3)}
\newcommand{\ensembleira}[3]{{\cal C}_{\text{IRA}} (#1,#2, #3)}
\newcommand{\ensemblesira}[3]{{\cal C}_{\text{SIRA}} (#1,#2, #3)}
\newcommand{\ensemblensira}[3]{{\cal C}_{\text{NSIRA}} (#1,#2, #3)}

% macros for graphs
\newcommand{\graphtextsizelarge}{\normal}
\newcommand{\graphtextsize}{\small}
\newcommand{\graphtextsizesmall}{\footnotesize}
\newcommand{\degd}{dd}
\newcommand{\azumaalpha}{\gamma}
\renewcommand{\mid}{\,|\,}

% formal power sums
% -----------------
\newcommand{\indet}{D}    % indeterminated of a formal power sum
\newcommand{\fps}{F}      % standard formal power sum
\newcommand{\fpstwo}{G}   % standard formal power sum
\newcommand{\fpsthree}{H} % standard formal power sum

% abbreviations for sub and superscripts
% --------------------------------------
\newcommand{\cw}{{\text{\myscriptsize cw}}}
\newcommand{\sss}{{\text{\myscriptsize ss}}}
\newcommand{\MAP}{{\text{\myscriptsize MAP}}}
\newcommand{\ML}{{\text{\myscriptsize ML}}}
\newcommand{\IT}{{\text{\myscriptsize IT}}}
\newcommand{\BP}{{\text{\myscriptsize BP}}}
\newcommand{\EXIT}{EXIT}
\newcommand{\GEXIT}{GEXIT}

